Writing in The Air: Unconstrained Text Recognition from Finger Movement Using Spatio-Temporal Convolution

In this paper, we introduce a new benchmark dataset for the challenging writing in the air (WiTA) task -- an elaborate task bridging vision and NLP. WiTA implements an intuitive and natural writing method with finger movement for human-computer interaction (HCI). Our WiTA dataset will facilitate the development of data-driven WiTA systems which thus far have displayed unsatisfactory performance -- due to lack of dataset as well as traditional statistical models they have adopted. Our dataset consists of five sub-datasets in two languages (Korean and English) and amounts to 209,926 video instances from 122 participants. We capture finger movement for WiTA with RGB cameras to ensure wide accessibility and cost-efficiency. Next, we propose spatio-temporal residual network architectures inspired by 3D ResNet. These models perform unconstrained text recognition from finger movement, guarantee a real-time operation by processing 435 and 697 decoding frames-per-second for Korean and English, respectively, and will serve as an evaluation standard. Our dataset and the source codes are available at https://github.com/Uehwan/WiTA.

==> 1_intro_backup.tex <==
\section{Introduction}\label{sec:introduction}
As new types of technologies such as mobile computing, AR and VR integrate into people’s daily lives, the need for a text entry system that suits the contemporary devices has emerged \cite{kim2019i}. Among various advanced text-entry methods, writing in the air (WiTA) in which people write letters or words with hand or finger movements in free space has drawn much attention \cite{zhang2013new}. An ideal WiTA system enables people to write text without focusing on tiny screens, and keyboard layouts and implements a natural and intuitive text-entry system. Applications that would benefit from WiTA and immensely improve the user experience with WiTA include automotive interfaces, remote signatures and smart system controls.

Developing feasible WiTA systems is challenging due to the interdependence among the involved gestures and lack of a concrete anchor or reference positions \cite{chen2015air}. As a result, the contemporary WiTA systems hardly achieve satisfactory performance for practical deployment into real-world applications. Conventional WiTA systems, in general, rely on traditional statistical models with hand-crafted features, which restricts their performance \cite{amma2014airwriting, mohammadi2019real}. Although researchers have attempted to apply data-driven approaches for the design of WiTA systems and to maximize the performance, there is no available benchmark dataset suitable for development and evaluation of WiTA systems to the best of our knowledge \cite{mukherjee2019fingertip}.

To overcome the limitations mentioned above, we first collect a benchmark dataset in this work. Among multiple modalities for capturing finger movements in the air, we select RGB cameras as the sensing device due to their superior accessibility, low cost, and generality compared to other sensing modalities such as depth or gyro sensors. Besides, we adopt a third-person view rather than an egocentric view to improve user experience by removing the possibility of attaching additional devices on users \cite{mukherjee2019fingertip}. Moreover, we collect five types of datasets in two languages (Korean and English) to ensure universality: Korean lexical, English lexical, Korean non-lexical, English non-lexical, and the mixture of the two languages in non-lexical format. As far as we are aware, our dataset is the first and the largest benchmark dataset for the WiTA task, and we expect our dataset would facilitate the research on WiTA within the corresponding research community.

Next, we propose baseline methods for the WiTA task, which will serve as an evaluation standard for forthcomping WiTA systems. The baseline methods receive a sequence of image frames and transform the input into a sequence of characters written in the air by users. The proposed baseline methods perform the decoding process in an end-to-end manner. In addition, we propose spatio-temporal residual network architectures inspired by 3D residual networks \cite{tran2018closer} in the process of developing the baseline methods. The proposed spatio-temporal residual networks effectively deal with both spatial and temporal contexts within the WiTA input signals. Besides, we conduct a thorough ablation study to examine the effect of each design choice and offer insights for the development of more advanced WiTA systems.

Specifically, the main contributions of our work are as follows.
\begin{enumerate}
\item \textbf{Benchmark Dataset}: We explicitly define the task of WiTA and collect five types of the dataset in two languages (Korean and English) for the development ans evaluation of WiTA systems.
\item \textbf{Baseline Methods}: We propose baseline methods for the WiTA task and propose saptio-temporal residual network architectures which translate an input video sequence into a sequence of characters written in the air.
\item \textbf{Ablation Study}: We conduct a comprehensive ablation study by varying the training conditions in multiple ways and analyze the effect of each design choice in a thorough manner.
\item \textbf{Open Source}: We contribute to the corresponding research society by making the source code of the data collection tool, the WiTA dataset, the proposed WiTA baseline networks and the pretrained network parameters public\footnote{\url{https://github.com/Uehwan/WiTA}}.
\end{enumerate}

The rest of this manuscript is structured as follows. Section II reviews previous research outcomes related to WiTA. Section III illustrates the data collection process and the data statistics. Section IV describes the proposed WiTA baseline networks and the training scheme. Section V delineates the evaluation setting and examines the evaluation results with corresponding analysis. Section VI discusses future research directions for further improvement of WiTA and concluding remarks follow in Section VII.
